Programming by Rewards

We formalize and study ``programming by rewards'' (PBR), a new approach for specifying and synthesizing subroutines for optimizing some quantitative metric such as performance, resource utilization, or correctness over a benchmark. A PBR specification consists of (1) input features $x$, and (2) a reward function $r$, modeled as a black-box component (which we can only run), that assigns a reward for each execution. The goal of the synthesizer is to synthesize a "decision function" $f$ which transforms the features to a decision value for the black-box component so as to maximize the expected reward $E[r \circ f (x)]$ for executing decisions $f(x)$ for various values of $x$. We consider a space of decision functions in a DSL of loop-free if-then-else programs, which can branch on linear functions of the input features in a tree-structure and compute a linear function of the inputs in the leaves of the tree. We find that this DSL captures decision functions that are manually written in practice by programmers. Our technical contribution is the use of continuous-optimization techniques to perform synthesis of such decision functions as if-then-else programs. We also show that the framework is theoretically-founded ---in cases when the rewards satisfy nice properties, the synthesized code is optimal in a precise sense. We have leveraged PBR to synthesize non-trivial decision functions related to search and ranking heuristics in the PROSE codebase (an industrial strength program synthesis framework) and achieve competitive results to manually written procedures over multiple man years of tuning. We present empirical evaluation against other baseline techniques over real-world case studies (including PROSE) as well on simple synthetic benchmarks.

==> eval_trees.tex <==
We now demonstrate that we can efficiently learn accurate trees, using Algorithm~\ref{alg:tree} for the common setting when $m = 1$, with black-box reward functions satisfying nice properties. Note that even if the reward function is concave (in decision value $a \in \mathbb{R}$), the resulting learning problem is still non-concave (because of the underlying neural network model $\fent$)  
%To this end, we consider synthetic parameter tuning problems with appropriate reward functions, where we know that the decisions can be optimally written as \texttt{if-then-else} construct, which maximizes the reward. 
To this end, we consider learning an ~\imp~decision function that has the~\textsc{Xor} structure, modeled on two features distributed as given in Figure~\ref{fig:xor.png} (in Appendix~\ref{app:evaluation}). We want to minimize the expected loss $\ell_{\text{sq}}$ defined in Equation~\eqref{eqn:loss} which is the squared error between the prediction and the actual value. The expectation, as in the results above, is with respect to the randomness in the features $x_1$ and $x_2$ that are uniformly sampled. We setup \selftune{} as: 

\ \ \ \ \texttt{XOR = \keywordc{lambda} x1, x2: \decfun(PBRID\_XOR, x1, x2);} \\
and the reward is assigned using:

\ \ \ \ \texttt{\assignr(-sqloss(XOR(x1, x2), expected(x1, x2))));}\\
Note that the reward is set as the negative of the computed~$\ell_{\text{sq}}$ loss (so as to maximize). The tree function for~\texttt{XOR} learnt by \selftune using Algorithm~\ref{alg:tree} with height $h = 2$ is given below. 
\begin{lstlisting}[escapechar=!,language=csh,morekeywords={public,static,double,return},basicstyle=\footnotesize\ttfamily]
double XOR(double x1, double x2) {
    if (x2 <= -0.02)
        if (x1 >= 0.04) return 0; else return 1;
    else
        if (x1 <= (-0.01 * x2 - 0.03)) return 0.03; else return 0.98;
}
\end{lstlisting}
On a close inspection, we see that the code effectively represents the expected function in Figure~\ref{fig:xor.png}. 
%Results for a more complex decision function requiring a tree of higher depth is presented in Appendix \ref{app:evaluation}.
%~In Figure~\ref{fig:xor_smart_vs_naive}, we compare the tree learning algorithm (Algorithm~\ref{alg:tree}) against learning the parameters of the tree by na\"ively treating them as constants using Algorithm~\ref{alg:constant}. As expected, we find that (a) our tree learning algorithm converges to the optimal reward, and (b) its sample complexity is much better as it exploits the template structure.


==> overview.tex <==
\section{Overview}
\label{sec:overview}
%Give an example end-to-end starting with how the operator is instantiated, how the data collection happens, how model learning works, and how the learnt model looks. 
This section gives a high-level, end-to-end overview of the \selftune\ operator, leaving 
%jg01 specifics and 
details to subsequent sections. It is helpful to walk through an example to keep the discussion of the operator semantics, problem formulation and learning details grounded. To this end, we will work with the code for the functions~\texttt{ScoreLinesMap} and~\texttt{isLikelyDataRatio} in Figure~\ref{fig:code-samples-prose}. 

\begin{figure}[h!]
\includegraphics[scale=0.3]{SelfTuneArch.PNG}\vspace*{-10pt}
\caption{\selftune\ architecture. The client interacts with the \selftune\ server via API specification discussed in Section~\ref{sec:API}. The learning happens on the server side, and it
is transparent to the client.\vspace*{-10pt}}
\label{fig:selftunearch}
\end{figure}

\selftune\ comprises (a) client API that enables developers/programmers to leverage machine learning/AI tools 
to create decision functions
%jg01: replace this with the above
%jg01 in specific parts of the code they deem essential for data-driven decision making, 
and (b) a service that provides the necessary AI tools. 
The client API is responsible for data collection while the server is responsible for learning ML models behind the scenes.  Figure~\ref{fig:selftunearch} depicts this architecture at a high-level. 

\subsection{\selftune{} interface} 
The client API of \selftune{} enables programmers to specify \textit{what} parts of the code or parameters they want to learn, \textit{how} they want to 
%jg01 learn 
%jg01: It is really learn or represent?
represent the learned rule (e.g., as an \texttt{if-then-else} rule that depends on some observed \textit{context} or \textit{features}), and how to supply feedback to the learning engine. 

\selftune{} carefully makes the trade-off between expressiveness and simplicity: We want 
an easy-to-use API that lets programmers express domain knowledge tightly in the code --- from the
{\emph template} for the decision variables, constraints on the parameters (e.g., their range) to be tuned, and features (typically, program variables or any other contextual information) that dictates the decision outcome. 
Our novel notion of templates for selecting the structure of the decision/control functions 
is critical as: a) it allows programmers to read, inspect, and possibly adjust the code that is 
generated by the learning algorithm, b) it allows the learning algorithm 
to exploit the structure to enable efficient solutions. 

%Note that it is important for the programmer to have visibility into the decision/control functions  --- it is essential to determine parameter values not with some black-box machine learning model (such as a neural network), but rather using an interpretable model.  

%should be able to  On one hand, we want the API to be simple and intuitive, and importantly, less demanding. On the other hand, it is important that the API lets programmers express domain knowledge tightly in the code --- such as constraints on the parameters (e.g. range) to be tuned, and features (typically, program variables or any other contextual information) that can help learn the parameter value. In addition, \selftune{} supports learning parameters in the form of interpretable code \textit{templates}. 


Figure~\ref{fig:code-samples-prose} illustrates two types of commonly used code templates 
%jg01: I commented this out
%for writing heuristics 
%to make some critical decisions in the code. 
for decision functions. In case of~\texttt{ScoreLinesMap}, the function value for is computed as a linear combination of its arguments; in case of~\texttt{IsLikelyDataRatio}, the function value is computed as a nested \texttt{if-then-else} construct. In machine learning parlance, the former is an example of a simple linear model and the latter is a decision tree model.  Table~\ref{tab:selftune} shows how the programmer can use \selftune{} to re-write the~\texttt{ScoreLinesMap} function (Figure~\ref{fig:code-samples-prose}) using a linear template. 
%\jg{Why is Templates.linear not red - isn't that a constant that indicates that we want to learn a linear function? And does our approach work beyond linear functions and decision trees?} 
The example in Table~\ref{tab:selftune} shows all the components of the client API. The API consists of (i) initializing the \selftune{} object, (ii) \Create{} interface for creating a new \selftune{} problem instance with details on the parameter to tune, (iii) \Connect{} interface connecting to the created (or an existing) problem instance, (iv) \Predict{} interface for getting predictions for the parameter values associated with the problem instance from the underlying machine learning model, and (v) \SetReward{} interface for giving feedback to the server side on the quality of the predictions. 

The use of templates for tuning parameter values is a distinguishing aspect of ~\selftune{}. Consider the alternative of using program sketching techniques~\cite{solar2006combinatorial} that try to fill in parts of some existing code/function. One could treat the hard-coded constants in the definition of~\texttt{ScoreLinesMap} as ``holes'', and rewrite the code using the \textsc{Sketch} language as shown below:

\begin{lstlisting}[language=dsl,morekeywords={public,static,double,return}]
double ScoreLinesMap(double selection, double lines) {
    double minScore = ??;double alpha = ??;double beta = ??;
    return alpha * selection + beta * lines + minScore * 20;
}
\end{lstlisting}\vspace*{-15pt}

The programmer can try to fill the holes (`??') by supplying an appropriate specification for the function. 
%\jg{Where does solving sketches come from -- was never mentioned before?}
But, the complexity of solving sketches grows exponentially with the number of holes we want to learn. In contrast,~\selftune{} provides new learning techniques which learn multiple real-valued parameters far more efficiently, using algorithms that exploit the special structure of the mapping from parameters and feature values to decisions, such  as linear functions or decision trees.
%Not only does it make the interface simple, but it also leads to a significant reduction in terms of sample complexity to learn the parameters, as we will see in Section~\ref{sec:learning}.

The programmer can create many such problem instances with desired templates (\selftune{} supports learning more complex templates like decision trees as described in Section~\ref{sec:learning}) --- multiple types of templates for different parameters can co-exist within the same code-base. At some point after the \Predict{} calls, the programmer needs to give feedback or \textit{reward} to~\selftune{} to indicate the quality of predictions. In the example of Table~\ref{tab:selftune}, a high positive reward is given when the predictions lead to successful completion of some task the code is meant for, or a high negative reward otherwise. 

%any constraints on them (e.g. range or type), and additional features or context that can help determine the values of the parameters; each problem instance has a persistent, globally unique identifier (variable \texttt{problemId} in Table~\ref{tab:selftune}), (b) \texttt{Predict} interface for getting predictions from the underlying ML model, and (c) \texttt{SetReward} interface for giving feedback to the server side on the quality of the predictions.
In practice, there are many aspects to consider when designing the operator; the details of syntax and semantics are given in Section~\ref{sec:API}. 

% \begin{table*}[ht]
%   \caption{\selftune\ Usage} \label{tab:selftune}
%   \begin{tabular}{l c l} \hline 
%      \textbf{(I) Initialize:}& & \texttt{\keywordc{var} st = \keywordc{new} SelfTune();} \\ 
%      & & \texttt{\keywordc{var} problemId = st.\stc{\textbf{Create}}(param: \stringc{``minScore''}}, \\
%     & & \ \ \texttt{constraints: \keywordc{new} Constraints(min: 0))}; \\
%     & & \texttt{st.Connect(problemId);} \\ \hline
%     \textbf{(II) Modify code:} & & \\
% 	\texttt{\keywordc{static double} ScoreAbsPos(\keywordc{double} k) \{} & & \texttt{\keywordc{static double} ScoreAbsPos(\keywordc{double} k) \{} \\ 
% 	\texttt{\ \ \ \ \keywordc{double} minScore = 100.0;} & $\xRightarrow{\hspace*{1.3cm}}$  & \texttt{\ \ \ \ \keywordc{double} minScore = st.\stc{\textbf{Predict}}(\stringc{``minScore''});} \\
%   \texttt{\ \ \ \ k = 1 / k - 1;} & & \texttt{\ \ \ \ k = 1 / k - 1;} \\ 
% 	\texttt{\ \ \ \ \keywordc{return} Math.Max(10 * minScore - } & & \texttt{\ \ \ \ \keywordc{return} Math.Max(10 * minScore - }\\
% 	\texttt{\ \ \ \ \ \ (k - 1) * 3 * minScore, 1 / k);} & &  \texttt{\ \ \ \ \ \ (k - 1) * 3 * minScore, 1 / k);}\\
% \texttt{\}}	& &  \texttt{\}} \\ \hline
%     \textbf{(III) Give feedback:} & & \texttt{st.\stc{\textbf{SetReward}}(succeeded ? +5: -5);}\\
%     \hline
%     \end{tabular}
% \end{table*}

% \begin{table*}[ht]
%   \caption{\selftune: \textsc{Sketch}-like usage (left) vs \textsc{Template} usage (right) for the function defined in Figure~\ref{fig:code-samples-prose}.} \label{tab:selftune}
%   \begin{tabular}{l | l} \hline 
%      \multicolumn{2}{l}{\textbf{(I) Initialize:} \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \texttt{\keywordc{var} st = \keywordc{new} SelfTune();}} \\ \hline
%      \textbf{(II) Create problem instance:} & \\
%     \texttt{\keywordc{var} problemId = st.\stc{\textbf{Create}}(param: \stringc{``minScore''}}, & \texttt{\keywordc{var} problemId = st.\stc{\textbf{Create}}(param: \stringc{``ScoreLinesMap''}},\\
%     \ \ \ \ \ \ \texttt{constraints: \keywordc{new} Constraints(min: 0))}; & \ \ \ \ \ \ \texttt{constraints: \keywordc{new} Constraints(min: 0), } \\
%     & \ \ \ \ \ \ \texttt{features:\{\stringc{``selection''}, \stringc{``lines''}\}, } \\ 
%     & \ \ \ \ \ \ \texttt{template: Templates.Linear); } \\ \hline
%      \multicolumn{2}{l}{\textbf{(III) Establish connection:} \ \ \ \ \ \ \ \ \ \texttt{st.\textbf{Connect}(problemId);}} \\ \hline
%     \textbf{(IV) Use prediction:} & \\
% 	\texttt{\keywordc{double} ScoreLinesMap(\keywordc{double} selection, \keywordc{double} lines)}  & \texttt{\keywordc{double} ScoreLinesMap(\keywordc{double} selection, \keywordc{double} lines) } \\ 
%     \texttt{\{} & \texttt{\{}\\
% 	\texttt{\ \ \ \ \keywordc{double} minScore = st.\stc{\textbf{Predict}}(\stringc{``minScore''});} &  \texttt{\ \ \ \ \keywordc{return} st.\stc{\textbf{Predict}}(\stringc{``ScoreLinesMap''},} \\
% 	\texttt{\ \ \ \ \keywordc{return} selection + lines + minScore * 20; }  & \texttt{\ \ \ \ \ \ \ \ \ \ \ \ \ selection: selection, lines: lines);}\\
%     \texttt{\}}	 &  \texttt{\}} \\ \hline
%      \multicolumn{2}{l}{\textbf{(IV) Give feedback:}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \texttt{st.\stc{\textbf{SetReward}}(succeeded ? +5: -5);}}\\
%     \hline
%     \end{tabular}
% \end{table*}

\begin{table*}[ht]
  \caption{\selftune: Implementing the function defined in Figure~\ref{fig:code-samples-prose} using an interpretable template.} \label{tab:selftune}
  \begin{tabular}{|l|l|} \hline 
     \textbf{(I) Initialize:} & \texttt{\keywordc{var} st = \keywordc{new} SelfTune();} \\ \hline
     \textbf{(II) Create problem instance:} &  \texttt{\keywordc{var} problemId = st.\stc{\textbf{Create}}(param: \stringc{``ScoreLinesMap''}},\\
    & \ \ \ \ \ \ \texttt{constraints: \keywordc{new} Constraints(min: 0), } \\
     & \ \ \ \ \ \ \texttt{features:\{\stringc{``selection''}, \stringc{``lines''}\}, } \\ 
     & \ \ \ \ \ \ \texttt{template: \textbf{Templates.Linear}); } \\ \hline
    \textbf{(III) Establish connection:} & \texttt{st.\stc{\textbf{Connect}}(problemId);} \\ \hline
    \textbf{(IV) Use prediction:} & \texttt{\keywordc{var} (invocationId, decision) =  st.\stc{\textbf{Predict}}(\{\stringc{``selection''}: selection,  \stringc{``lines''}: lines\});}\\
    \hline
    \textbf{(V) Give feedback:} & \texttt{st.\stc{\textbf{SetReward}}(invocationId, succeeded ? +5: -5);}\\
    \hline
    \end{tabular}
\end{table*}

\subsection{Data logging and tracking rewards}
Every time the client makes a \Predict{} call, with optional arguments/features $\featvals = (\featval_1, \featval_2, \dots, \featval_\numcontext)$, it gets back a decision (or \textit{action}~\cite{agarwal2016multiworld}), say $\paramval \in \mathbb{R}$, for the parameter associated with the problem instance; more generally, it gets back a vector of $\numparam$ decisions connected to the~\selftune{} object. In the example of Table~\ref{tab:selftune}, there is one decision variable  \texttt{ScoreLinesMap}, and there are two associated features~\texttt{selection} and~\texttt{lines} whose values are logged during the~\Predict{} call. \Predict{} returns a pair of values: (1) the first value is an unique identifier to refer to the specific invocation of \Predict, and (2) the second value is the decision value. The \selftune{} backend maintains a persistent store for the decisions given to the client against the corresponding problem instance id and features.

Whenever the client makes a subsequent call to \SetReward{} interface, with a value $r$, the reward is associated with the particular problem instance, and in particular, the invocation of \Predict{} (identified using \texttt{invocationId} in Table~\ref{tab:selftune}); recall that the reward is the value of some key metric that the developer wants to maximize by setting the decision function appropriately. So, the reward tracker in the backend is responsible for updating the store with the tuples of the form $(\featvals, \paramval, r)$ against the corresponding problem instance. This can be tricky because, in many settings, the rewards arrive \textit{asynchronously} and much later (even days) than the corresponding decisions. The data thus collected must be used by the learning engine in the server-side for updating the corresponding models. 

\subsection{Learning}
\begin{figure}[h!]
\includegraphics[scale=0.3]{raw.PNG}\vspace*{-10pt}
\caption{Decisions $\paramvals$ given to the client are modeled as a function of parameters $\weights$, and rewards are computed for the given decisions $\paramvals$.}\vspace*{-10pt}
\label{fig:raw}
\end{figure}
The goal is to learn the parameters and hence the decision functions that would  maximize the developer-supplied reward over time. Algorithm~\ref{alg:basic} shows how~\selftune{} learns continuously in rounds. Step 6 in Algorithm~\ref{alg:basic} uses the collected data to learn/update the underlying ML model. The key challenge here is that one cannot directly invoke classical optimization algorithms (like gradient-descent) because the reward function is unknown; the reward function in general can be too complicated to even write down, and importantly, ~\selftune{} only has \emph{blackbox} access to rewards, i.e., it obtains the value of $r$ for a given decision variable $\paramval$, but no other information regarding the reward function is revealed. We can, however, estimate the gradient using  standard perturbation  techniques~\cite{flaxman2005online} and by exploiting the structure in our templates.  This technique naturally extends to settings where multiple decisions need to be made simultaneously (i.e. $\paramvals^{(t)}$ is a vector). So, the learner updates the parameters in the direction of the negative gradient, gets reward for the updated parameter(s), and repeats until some notion of convergence. We show that this  simple algorithm has rigorous guarantees under some assumptions on the reward function, and in certain cases is able to significantly improve state-of-the-art results (see Section~\ref{sec:learning}). For example, our technique is able to ensure that the regret scales only with {\em size of decision variables} ($m$) instead of the total number of parameters ($d$) which can be significantly larger (typically $m \leq 10$ while $d$ can be $\geq 100$). Finally, while assumptions on reward functions (such as convexity) are needed in theory for proving the convergence, the technique works well for general reward functions arising in practice. 

%There are variants of this basic problem formulation and algorithm, depending on the availability of features, which in turn influences the choice of prediction model $g$ and Step~6 of Algorithm~\ref{alg:basic}. If no context is available, then the parameters can be simply treated as constants (\texttt{Templates.Constant}); otherwise, interpretable templates are available for making decisions: (a) linear $g$, where the decision is a linear function of the features, or (b) tree model, where the decision is made using \texttt{if-then-else} construct.
\begin{algorithm}
\caption{Pseudocode for learning in~\selftune{}}\label{alg:basic}
\begin{algorithmic}[1]
\Procedure{LearnInRounds}{}
\State Initialize the prediction model $g^{(0)}$ \stc{//\ \textbf{\texttt{Create}}}
\For{$t = 0,1,2,\dots$}
\State Client receives decision $\paramval^{(t)} := g^{(t)}(.)$  \stc{//\ \textbf{\texttt{Predict}}}
\State Receive feedback $r^{(t)}$  \stc{//\ \textbf{\texttt{SetReward}}}
\State Update $g^{(t+1)}$ using $(\paramval^{(t)}, r^{(t)})$
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

%In Section~\ref{sec:learning}, we show how we can exploit the problem structure resulting from the use of simple templates, to devise variants of the basic gradient-descent style optimization algorithm outlined above. In particular, we show, under certain assumptions, that the proposed algorithms have better convergence guarantees (i.e., significantly fewer reward computations to find the optimal solution) than state-of-the-art techniques to solve the problem.

\subsection{Deployment} When the code in Table~\ref{tab:selftune} is checked in and built, the training of the model effectively starts. The developer need not set aside time nor oversee the training process. It happens transparently, whenever the code is executed (say, via nightly builds which are common in code management repositories). The developer can then query decision outcomes from the trained model (using the \Predict{} API), get the expression tree for the model (using the \GetExprTree{} API discussed in Section~\ref{sec:API}), which generates interpretable code to inspect, as well as explicitly control when the model should be updated via the \Refresh{} API. At deployment, the developer can either continue to use the trained model and choose not to invoke \Refresh{}, or continue to update the model at a determined frequency in an online fashion.

==> validation.tex <==
\subsection{Do our algorithms compute optimal parameters when the black-box reward function satisfies nice properties?}
\label{sec:validation}
The goal of this study is to verify that our algorithms indeed compute the optimal parameters when the black-box reward function $r$ satisfies the properties required for the theoretical guarantees to hold (say, Theorem~\ref{thm:linear}) including concavity and Lipschitz continuity. In particular, we measure the ability to learn accurate solutions with small sample complexity as well within a given time budget. We compare \selftune{} with the~\sketch{} synthesis tool~\cite{sketchtool} and a black box optimization algorithm implemented in the open-source \Nevergrad platform~\cite{nevergrad}. Specifically, we use TBPSA, an evolutionary algorithm that can perform well in continuous, stochastic settings~\cite{tbpsa}. Note that \textit{all the compared algorithms have only black-box access to the reward function}. 
%a sketching-based program synthesis technique~\cite{solar2006combinatorial} and 
%a representative multi-arm bandit algorithm~\cite{Auer2002} used in~\decisionservice~\cite{agarwal2016multiworld}, an enterprise-standard reinforcement learning framework for online decision making in software and services. For program synthesis, we use the~\sketch{} synthesis tool~\cite{sketchtool} that relies on CEGIS solver in the backend. For the multi-arm bandit algorithm, we use the popular Vowpal Wabbit (VW) library~\citet{VW}.

The~\sketch{} tool suffers from two key limitations: (a) it is prohibitively expensive in terms of time as well as of memory even when the number of parameters (which are modeled using holes) increases beyond 5, (b) it works with integer holes and computations only.
%; extensions to floating point programs is still an open area of research. 
Due to these limitations, we work with simple low-dimensional synthetic problems where we have defined simple reward functions that satisfy the required properties. In practice, the reward function is unknown, highly complex and noisy, but the results below show that our algorithms outperform sketching even in this simple setting. In the more complicated settings (studied in subsequent sections), we cannot run sketch due to limitations mentioned above. 

\begin{remark}
% For this study, we restrict the problems to be integral because extending state-of-the-art sketching techniques to floating point computations can further increase the sample and computational complexity of the system. 
Sketching techniques that handle real-valued parameter synthesis, e.g.~\cite{chaudhuri2014bridging}, do not apply to the problem instances we consider here, especially because they require black-box rewards (see Section~\ref{sec:whitebox} for a different study). 
\end{remark}

We generate problems of the following type, where the goal is to learn a~\implin~decision function $f(\cdot; \weights)$, with integral $\weights \in \mathbb{Z}^d$, such that the following expected reward is maximized:
% \begin{equation}
%     \min_{\weights \in \mathbb{Z}^\numfeat} L(\weights) = \sum_{i=1}^\numex \ell\big(\langle \weights, \featvals^{(i)}\rangle\big),
% \label{eqn:toyproblem}
% \end{equation}
\begin{equation}
    \max_{\weights \in \mathbb{Z}^\numfeat} \mathbb{E}[r\big( \weights \cdot \featvals \big)],
\label{eqn:toyproblem}
\end{equation} 
where the expectation is with respect to randomness in the features $\featvals$ and the reward $r(.)$ is set to be negative of loss $\ell$ (minimizing the loss is equivalent to maximizing the reward), defined below:
\begin{align}
\label{eqn:loss}
\ell_{\text{sq}}(y) := \big(y - y^{*}\big)^2, \text{ or } \ell_{\text{abs}}(y) := \big|y - y^{*}\big|. 
\end{align}
The values $y^{*}$ are chosen to be such that $y^{*} =  \weights^* \cdot \featvals$ for some fixed $\weights^* \in [0,1,2,\dots,10]^\numfeat$ which is the optimal solution to the problem~\eqref{eqn:toyproblem}. We assume a uniform distribution over $n$ features $\x$ to compute the expectation in ~\eqref{eqn:toyproblem}. We fix $n = 2d$ in all cases (which is sufficient for learning).

%The pseudo-code for implementing the optimization problem~\eqref{eqn:toyproblem} in \sketch{} is given in Algorithm~\ref{alg:sketch}. 
The \sketch{} implementation is given in Figure~\ref{fig:code-sketch} (Appendix~\ref{app:evaluation:sketch}). For~\selftune{}, we use Algorithm~\ref{alg:linear} (fixing $\delta = 0.5$ and $\eta = 2\times10^{-3}$) meant for~\implin~decision functions. %\red{change UCB to \Nevergrad/TBPSA here}
%and for the multi-arm bandit formulation we use the Upper Confidence Bound algorithm (\textsc{UCB}) with the action space $[0,1,\dots,10]^d$. 

\begin{remark}
We restrict the search space for~\sketch{} further by ensuring that $\weights^*$ values are non-negative (requirement of the tool), small and bounded; we explicitly add these bound constraints in the ~\sketch{} problem specification. See the \texttt{assert}ion in Figure~\ref{fig:code-sketch}. Furthermore, in all the experiments, we work with 4-bit integers for holes, which we know is sufficient, using the flag \texttt{bnd-cbits} in the~\sketch{} tool. Using larger-sized integers will only increase the computation time.
\end{remark}

We create multiple problem sets varying number of parameters $\numfeat$ in Equation~\eqref{eqn:toyproblem}. To account for randomness in algorithms as well as in problem sets themselves, we repeat each experiment 10 times and report (a) accuracy, i.e. how often does the method solve the problem~\eqref{eqn:toyproblem} exactly, and (b) mean and standard deviation of time taken to solve. Results are presented in~Table~\ref{tab:sketch}, for the two loss functions given in~\eqref{eqn:loss}. It is clear that the search algorithm of sketching takes prohibitively long time, and fails to solve the problem even for small values of $d$ within the budget of 1 hour (and in many cases, we find that the tool prematurely fails well before the timeout despite multiple restarts with random seeds). In case of squared loss $\ell_{\text{sq}}$, sketching totally fails because it involves using multiplication circuits in the back-end SAT problem. Our algorithm solves every problem instance (as guaranteed by Theorem~\ref{thm:linear}). Even the general-purpose, continuous, black-box optimization algorithm of~\Nevergrad{} fails to compute the exact solution in most of the cases within 1 hour. The progress of \Nevergrad{} and~\selftune{} algorithms against \# reward queries is shown in Figure~\ref{fig:sketchcomp}. 

\begin{table*}[t]
\caption{Comparison of techniques on parameter learning problem in Equation~\eqref{eqn:toyproblem}, for the two losses defined in Equation~\eqref{eqn:loss}, for increasing number of parameters (holes) $\numfeat$. The implementation of~\sketch{} is given in Figure~\ref{fig:code-sketch}. For each $d$, we create 10 problem sets and report the mean and the standard deviation of the time taken (in seconds) to solve the problems. %For each configuration of $d$ and $n$, we create 10 problem sets and report the mean and the standard deviation of the time taken (in seconds) to solve the problems. 
The number of cases successfully solved out of 10 is indicated in parentheses. Timeout is set to 1 hour.}
\label{tab:sketch}
\begin{center}
\begin{footnotesize}
% \begin{tabular}{cc|rrr|rrr}
% \toprule
% $d$ & $n$ & \multicolumn{3}{c|}{$\ell_{\text{abs}}$} & \multicolumn{3}{c}{$\ell_{\text{sq}}$}\\ \hline
% & & \sketch & \selftune & UCB & \sketch & \selftune & UCB \\
% \hline
% 2  & 2 & 0.40 $\pm$ 0.02 (\good{10}) & 0.98 $\pm$ 0.90 (\good{10}) & 0.01 $\pm$ 0.01 (\good{10}) & 1.59 $\pm$ 1.18 (\good{10}) & 3.49 $\pm$ 8.97 (\good{10}) & 0.01 $\pm$ 0.00 (\good{10})\\
%   & 4 & 0.49 $\pm$ 0.04 (\good{10}) & 0.42 $\pm$ 0.12 (\good{10}) & 0.02 $\pm$ 0.01 (\good{10}) & 70.8 $\pm$ 73.95 (\good{10}) & 0.20 $\pm$ 0.04 (\good{10}) & 0.01 $\pm$ 0.00 (\good{10}) \\ \hline
% 4  & 4 & 2.72 $\pm$ 1.89 (\good{10}) & 1.09 $\pm$ 0.59 (\good{10}) & 4.39 $\pm$ 2.84 (\good{10}) & - (\bad{0}) & 1.52 $\pm$ 2.39 (\good{10}) & 3.14 $\pm$ 1.96 (\good{10}) \\
%   & 8 & 9.65 $\pm$ 7.72 (\good{10}) & 0.38 $\pm$ 0.06 (\good{10}) & 3.95 $\pm$ 2.06 (\good{10}) & - (\bad{0}) & 0.22 $\pm$ 0.03 (\good{10}) & 3.08 $\pm$ 1.84 (\good{10}) \\ \hline
% 6  & 6 & 496.4 $\pm$ 516.6 (\bad{3}) & 1.16 $\pm$ 0.84 (\good{10}) & - (\bad{0}) & - (\bad{0})& 0.54 $\pm$ 0.26 (\good{10}) & 530.7 $\pm$ 0.0 (\bad{1})\\
%   & 12 & 582.1 $\pm$ 425.0 (\bad{5}) & 0.52 $\pm$ 0.09 (\good{10}) & - (\bad{0}) &- (\bad{0}) & 0.24 $\pm$ 0.05 (\good{10}) & - (\bad{0})\\ \hline
% 8  & 8 & 1103.1 $\pm$ 32.55 (\bad{2}) & 3.36 $\pm$ 4.32 (\good{10}) & - (\bad{0}) & - (\bad{0})& 3.56 $\pm$ 7.34 (\good{10}) & - (\bad{0})\\
%   & 16 & - (\bad{0})  & 0.50 $\pm$ 0.11 (\good{10}) & - (\bad{0}) & - (\bad{0})& 0.27 $\pm$ 0.06 (\good{10}) & - (\bad{0})\\ 
% % 10  & 10 & - (\bad{0})  & $\pm$ & $\pm$ &- (\bad{0})& & \\
% %   & 20 & - (\bad{0})  & $\pm$ & $\pm$ &- (\bad{0}) & & \\
% \bottomrule
% \end{tabular}
% \begin{tabular}{cc|rrr|rrr}
% \toprule
% $d$ & $n$ & \multicolumn{3}{c|}{$\ell_{\text{abs}}$} & \multicolumn{3}{c}{$\ell_{\text{sq}}$}\\ \hline
% & & \sketch & \selftune & \Nevergrad & \sketch & \selftune & \Nevergrad \\
% \hline
% 2  & 2 & 0.40 $\pm$ 0.02 (\good{10}) & 0.09 $\pm$ 0.09 (\good{10}) & - (\bad{0}) & 1.59 $\pm$ 1.18 (\good{10}) & 0.30 $\pm$ 0.82 (\good{10}) & 0.15 $\pm$ 0 (\bad{1})\\
%   & 4 & 0.49 $\pm$ 0.04 (\good{10}) & 0.04 $\pm$ 0.01 (\good{10}) & 298.66 $\pm$ 555.73 (\bad{5}) & 70.8 $\pm$ 73.95 (\good{10}) & 0.01 $\pm$ 0.00 (\good{10}) & 0.41 $\pm$ 0.15 (\bad{3}) \\ \hline
% 4  & 4 & 2.72 $\pm$ 1.89 (\good{10}) & 0.11 $\pm$ 0.07 (\good{10}) & - (\bad{0}) & - (\bad{0}) & 0.12 $\pm$ 0.19 (\good{10}) & - (\bad{0}) \\
%   & 8 & 9.65 $\pm$ 7.72 (\good{10}) & 0.04 $\pm$ 0.01 (\good{10}) & - (\bad{0}) & - (\bad{0}) & 0.01 $\pm$ 0.00 (\good{10}) & - (\bad{0}) \\ \hline
% 6  & 6 & 496.4 $\pm$ 516.6 (\bad{3}) & 0.13 $\pm$ 0.09 (\good{10}) & - (\bad{0}) & - (\bad{0})& 0.04 $\pm$ 0.03 (\good{10}) & - (\bad{0})\\
%   & 12 & 582.1 $\pm$ 425.0 (\bad{5}) & 0.07 $\pm$ 0.03 (\good{10}) & - (\bad{0}) &- (\bad{0}) & 0.01 $\pm$ 0.00 (\good{10}) & - (\bad{0})\\ \hline
% 8  & 8 & 1103.1 $\pm$ 32.55 (\bad{2}) & 0.31 $\pm$ 0.34 (\good{10}) & - (\bad{0}) & - (\bad{0})& 0.19 $\pm$ 0.35 (\good{10}) & - (\bad{0})\\
%   & 16 & - (\bad{0})  & 0.06 $\pm$ 0.02 (\good{10}) & - (\bad{0}) & - (\bad{0})& 0.02 $\pm$ 0.01 (\good{10}) & - (\bad{0})\\ 
% % 10  & 10 & - (\bad{0})  & $\pm$ & $\pm$ &- (\bad{0})& & \\
% %   & 20 & - (\bad{0})  & $\pm$ & $\pm$ &- (\bad{0}) & & \\
% \bottomrule
% \end{tabular}
\begin{tabular}{c|r|r|r|r|r|r}
\toprule
$d$ & \multicolumn{3}{c|}{$\ell_{\text{abs}}$} & \multicolumn{3}{c}{$\ell_{\text{sq}}$}\\ \hline
 & \sketch & \selftune (Alg.~\ref{alg:linear})& \Nevergrad & \sketch & \selftune (Alg.~\ref{alg:linear}) & \Nevergrad \\
\hline
 2 & 0.49 $\pm$ 0.04 (\good{10}) & 0.04 $\pm$ 0.01 (\good{10}) & 298.66 $\pm$ 555.73 (\bad{5}) & 70.8 $\pm$ 73.95 (\good{10}) & 0.01 $\pm$ 0.00 (\good{10}) & 0.41 $\pm$ 0.15 (\bad{3}) \\ 
 4 & 9.65 $\pm$ 7.72 (\good{10}) & 0.04 $\pm$ 0.01 (\good{10}) & - (\bad{0}) & - (\bad{0}) & 0.01 $\pm$ 0.00 (\good{10}) & - (\bad{0}) \\ 
 6 & 582.1 $\pm$ 425.0 (\bad{5}) & 0.07 $\pm$ 0.03 (\good{10}) & - (\bad{0}) &- (\bad{0}) & 0.01 $\pm$ 0.00 (\good{10}) & - (\bad{0})\\ 
 8 & - (\bad{0})  & 0.06 $\pm$ 0.02 (\good{10}) & - (\bad{0}) & - (\bad{0})& 0.02 $\pm$ 0.01 (\good{10}) & - (\bad{0})\\ 
% 10  & 10 & - (\bad{0})  & $\pm$ & $\pm$ &- (\bad{0})& & \\
%   & 20 & - (\bad{0})  & $\pm$ & $\pm$ &- (\bad{0}) & & \\
\bottomrule
\end{tabular}
\end{footnotesize}
\end{center}
\end{table*}

\begin{figure}[t]
\begin{tabular}{cc}
\hspace*{-10pt}\includegraphics[width=.51\linewidth]{exps_imgs/ng-st-sketch-d2.png}&
\hspace*{-10pt}\includegraphics[width=.51\linewidth]{exps_imgs/ng-st-sketch-d8.png}\\
(a) Squared loss $\ell_{\text{sq}}$ & (b) Abs. deviation loss $\ell_{\text{abs}}$
\end{tabular}
\caption{Expected reward (in problem~\eqref{eqn:toyproblem}) vs. number of queries to reward $r$ for loss functions in Equation~\eqref{eqn:loss}.}
\label{fig:sketchcomp}
\end{figure}

We tried to relax the sketch specification to not require exact solution to problem~\eqref{eqn:toyproblem} but approximate to a small additive error; however, the sketch tool still fails (See Appendix~\ref{app:evaluation:sketch}).

\input{eval_trees}
